Hibernate Container: A Deflated Container Mode for Fast Startup and High-density Deployment in Serverless Computing

Serverless computing is a popular cloud computing paradigm, which requires low response latency to handle on-demand user requests. There are two prominent techniques employed for reducing the response latency: keep fully initialized containers alive (Warm Container) or reduce the new container startup (cold start) latency. This paper presents the 3rd container startup mode: Hibernate Container, which starts faster than the cold start container mode and consumes less memory than the Warm Container mode. Hibernate Container is essentially a "deflated" Warm Container. Its application memory is swapped out to disk, the freed memory is reclaimed and file based mmap memory is cleaned-up. The Hibernate Container's deflated memory is inflated in response to user requests. As Hibernate Container's application is fully initialized, its response latency is less than the cold start mode; and as the application memory is deflated, its memory consumption is less than the Warm Container mode. Additionally, when a Hibernate Container is "woken up" to process a request, the Woken-up Container has similar response latency to Warm Container but less memory consumption because not all the deflated memory needs to be inflated. We implemented the Hibernate technique as part of the open source Quark secure container runtime project and our test demonstrated that Hibernate Container consumes about 7\% to 25\% of the Warm Container memory. All of this results in a higher deployment density, lower latency and appreciable improvements in the overall system performance.

==> temp.tex <==
@MISC{Fargate,
  title = {{AWS Fargate}},
  author = {},
  howpublished = {\url{https://docs.aws.amazon.com/whitepapers/latest/architecting-hipaa-security-and-compliance-on-aws/aws-fargate.html}},
  year = {2022}
}

@MISC{gVisor,
  title = {{Google gVisor: Container Runtime Sandbox}},
  author = {},
  howpublished = {\url{https://github.com/google/gvisor}},
  year = {2022}
}

@MISC{cloudfunction,
  title = {{Google Cloud Function}},
  author = {},
  howpublished = {\url{https://cloud.google.com/ functions}},
  year = {2022}
}

@MISC{cloudrun,
  title = {{Google Cloud Run}},
  author = {},
  howpublished = {\url{https://cloud.google.com/run/}},
  year = {2022}
}

@MISC{azurefunction,
  title = {{Azure Functions documentation}},
  author = {},
  howpublished = {\url{https://azure.microsoft.com/en-us/products/container-instances/\#overview}},
  year = {2022}
}

@MISC{azurecontainer,
  title = {{Azure container instances}},
  author = {},
  howpublished = {\url{https://learn.microsoft.com/en-us/azure/azure-functions/}},
  year = {2022}
}

@MISC{quark,
  title = {{Quark Container: A secure container runtime with OCI interface}},
  author = {},
  howpublished = {\url{https://github.com/QuarkContainer/Quark}},
  year = {2022}
}

@inproceedings{shahrad2020serverless,
  title={Serverless in the wild: Characterizing and optimizing the serverless workload at a large cloud provider},
  author={Shahrad, Mohammad and Fonseca, Rodrigo and Goiri, {\'I}{\~n}igo and Chaudhry, Gohar and Batum, Paul and Cooke, Jason and Laureano, Eduardo and Tresness, Colby and Russinovich, Mark and Bianchini, Ricardo},
  booktitle={2020 USENIX Annual Technical Conference (USENIX ATC 20)},
  pages={205--218},
  year={2020}
}

@MISC{optane,
  title = {{Google Cloud}},
  author = {},
  howpublished = {\url{https://cloud.google.com/blog/topics/partners/available-first-on-google-cloud-intel-optane-dc-persistent-memory}},
  year = {2022}
}

@MISC{CouldFlare,
  title = {{Cloudflare Docs - Cloudflare worker security model,}},
  author = {},
  howpublished = {\url{https://developers.cloudflare.com/workers/learning/security-model/}},
  year = {2022}
}

@inproceedings{RunD,
  title={$\{$RunD$\}$: A Lightweight Secure Container Runtime for High-density Deployment and High-concurrency Startup in Serverless Computing},
  author={Li, Zijun and Cheng, Jiagan and Chen, Quan and Guan, Eryu and Bian, Zizheng and Tao, Yi and Zha, Bin and Wang, Qiang and Han, Weidong and Guo, Minyi},
  booktitle={2022 USENIX Annual Technical Conference (USENIX ATC 22)},
  pages={53--68},
  year={2022}
}

@MISC{kata,
  title = {{Kata containers - open source container runtime software}},
  author = {},
  howpublished = {\url{https://katacontainers.io/}},
  year = {2022}
}

@inproceedings{agache2020firecracker,
  title={Firecracker: Lightweight virtualization for serverless applications},
  author={Agache, Alexandru and Brooker, Marc and Iordache, Alexandra and Liguori, Anthony and Neugebauer, Rolf and Piwonka, Phil and Popa, Diana-Maria},
  booktitle={17th USENIX symposium on networked systems design and implementation (NSDI 20)},
  pages={419--434},
  year={2020}
}

@inproceedings{oakes2018sock,
  title={$\{$SOCK$\}$: Rapid task provisioning with $\{$Serverless-Optimized$\}$ containers},
  author={Oakes, Edward and Yang, Leon and Zhou, Dennis and Houck, Kevin and Harter, Tyler and Arpaci-Dusseau, Andrea and Arpaci-Dusseau, Remzi},
  booktitle={2018 USENIX Annual Technical Conference (USENIX ATC 18)},
  pages={57--70},
  year={2018}
}

@inproceedings{ustiugov2021benchmarking,
  title={Benchmarking, analysis, and optimization of serverless function snapshots},
  author={Ustiugov, Dmitrii and Petrov, Plamen and Kogias, Marios and Bugnion, Edouard and Grot, Boris},
  booktitle={Proceedings of the 26th ACM International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={559--572},
  year={2021}
}

@inproceedings{du2020catalyzer,
  title={Catalyzer: Sub-millisecond startup for serverless computing with initialization-less booting},
  author={Du, Dong and Yu, Tianyi and Xia, Yubin and Zang, Binyu and Yan, Guanglu and Qin, Chenggang and Wu, Qixuan and Chen, Haibo},
  booktitle={Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={467--481},
  year={2020}
}

@article{amit2014vswapper,
  title={Vswapper: A memory swapper for virtualized environments},
  author={Amit, Nadav and Tsafrir, Dan and Schuster, Assaf},
  journal={Acm Sigplan Notices},
  volume={49},
  number={4},
  pages={349--366},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@inproceedings{gu2017efficient,
  title={Efficient memory disaggregation with infiniswap},
  author={Gu, Juncheng and Lee, Youngmoon and Zhang, Yiwen and Chowdhury, Mosharaf and Shin, Kang G},
  booktitle={14th USENIX Symposium on Networked Systems Design and Implementation (NSDI 17)},
  pages={649--667},
  year={2017}
}

@inproceedings{salomie2013application,
  title={Application level ballooning for efficient server consolidation},
  author={Salomie, Tudor-Ioan and Alonso, Gustavo and Roscoe, Timothy and Elphinstone, Kevin},
  booktitle={Proceedings of the 8th ACM European Conference on Computer Systems},
  pages={337--350},
  year={2013}
}

@article{liu2014hotplug,
  title={Hotplug or ballooning: A comparative study on dynamic memory management techniques for virtual machines},
  author={Liu, Haikun and Jin, Hai and Liao, Xiaofei and Deng, Wei and He, Bingsheng and Xu, Cheng-zhong},
  journal={IEEE Transactions on parallel and distributed systems},
  volume={26},
  number={5},
  pages={1350--1363},
  year={2014},
  publisher={IEEE}
}

@inproceedings{fuerst2022memory,
  title={Memory-harvesting vms in cloud platforms},
  author={Fuerst, Alexander and Novakovi{\'c}, Stanko and Goiri, {\'I}{\~n}igo and Chaudhry, Gohar Irfan and Sharma, Prateek and Arya, Kapil and Broas, Kevin and Bak, Eugene and Iyigun, Mehmet and Bianchini, Ricardo},
  booktitle={Proceedings of the 27th ACM International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={583--594},
  year={2022}
}

@article{liu2017effectively,
  title={Effectively mitigating cross-VM side-channel attacks by re-designing the hypervisor’s scheduler},
  author={Liu, Li and Wang, An and Chen, Songqing},
  year={2017}
}

@article{zhang2014mitigating,
  title={On mitigating the risk of cross-VM covert channels in a public cloud},
  author={Zhang, Rui and Su, Xiaojun and Wang, Jianping and Wang, Cong and Liu, Wenyin and Lau, Rynson WH},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={26},
  number={8},
  pages={2327--2339},
  year={2014},
  publisher={IEEE}
}

@article{wu2014whispers,
  title={Whispers in the hyper-space: high-bandwidth and reliable covert channel attacks inside the cloud},
  author={Wu, Zhenyu and Xu, Zhang and Wang, Haining},
  journal={IEEE/ACM Transactions on Networking},
  volume={23},
  number={2},
  pages={603--615},
  year={2014},
  publisher={IEEE}
}

@inproceedings{fuerst2021faascache,
  title={FaasCache: keeping serverless computing alive with greedy-dual caching},
  author={Fuerst, Alexander and Sharma, Prateek},
  booktitle={Proceedings of the 26th ACM International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={386--400},
  year={2021}
}

@inproceedings{kim2019functionbench,
  title={Functionbench: A suite of workloads for serverless cloud function service},
  author={Kim, Jeongchul and Lee, Kyungyong},
  booktitle={2019 IEEE 12th International Conference on Cloud Computing (CLOUD)},
  pages={502--504},
  year={2019},
  organization={IEEE}
}

@MISC{madvise,
  title = {{madvise}},
  author = {},
  howpublished = {\url{https://man7.org/linux/man-pages/man2/madvise.2.html}},
  year = {2022}
}

@article{knowlton1965fast,
  title={A fast storage allocator},
  author={Knowlton, Kenneth C},
  journal={Communications of the ACM},
  volume={8},
  number={10},
  pages={623--624},
  year={1965},
  publisher={ACM New York, NY, USA}
}

@MISC{rust,
  title = {{Rust Atomic}},
  author = {},
  howpublished = {\url{https://doc.rust-lang.org/stable/core/sync/atomic/}},
  year = {2022}
}

@inproceedings{zhang2016return,
  title={Return-oriented flush-reload side channels on arm and their implications for android devices},
  author={Zhang, Xiaokuan and Xiao, Yuan and Zhang, Yinqian},
  booktitle={Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security},
  pages={858--870},
  year={2016}
}

@inproceedings{gullasch2011cache,
  title={Cache games--bringing access-based cache attacks on AES to practice},
  author={Gullasch, David and Bangerter, Endre and Krenn, Stephan},
  booktitle={2011 IEEE Symposium on Security and Privacy},
  pages={490--505},
  year={2011},
  organization={IEEE}
}

@MISC{FirecrackerRecommand,
  title = {{Production Host Setup Recommendations}},
  author = {The Firecracker Authors},
  howpublished = {\url{https://github.com/firecracker-microvm/firecracker/blob/master/docs/prod-host-setup.md}},
  year = {2022}
}

@article{mitigating,
  title={On mitigating the risk of cross-VM covert channels in a public cloud},
  author={Zhang, Rui and Su, Xiaojun and Wang, Jianping and Wang, Cong and Liu, Wenyin and Lau, Rynson WH},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={26},
  number={8},
  pages={2327--2339},
  year={2014},
  publisher={IEEE}
}

@inproceedings{Catalyzer,
  title={Catalyzer: Sub-millisecond startup for serverless computing with initialization-less booting},
  author={Du, Dong and Yu, Tianyi and Xia, Yubin and Zang, Binyu and Yan, Guanglu and Qin, Chenggang and Wu, Qixuan and Chen, Haibo},
  booktitle={Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={467--481},
  year={2020}
}

@inproceedings{Recycle,
  title={Help Rather Than Recycle: Alleviating Cold Startup in Serverless Computing Through $\{$Inter-Function$\}$ Container Sharing},
  author={Li, Zijun and Guo, Linsong and Chen, Quan and Cheng, Jiagan and Xu, Chuhao and Zeng, Deze and Song, Zhuo and Ma, Tao and Yang, Yong and Li, Chao and others},
  booktitle={2022 USENIX Annual Technical Conference (USENIX ATC 22)},
  pages={69--84},
  year={2022}
}

@inproceedings{replayable,
  title={Replayable execution optimized for page sharing for a managed runtime environment},
  author={Wang, Kai-Ting Amy and Ho, Rayson and Wu, Peng},
  booktitle={Proceedings of the Fourteenth EuroSys Conference 2019},
  pages={1--16},
  year={2019}
}
